YellowFin and the Art of Momentum Tuning

Hyperparameter tuning is one of the most time-consuming workloads in deep learning. State-of-the-art optimizers, such as AdaGrad, RMSProp and Adam, reduce this labor by adaptively tuning an individual learning rate for each variable. Recently researchers have shown renewed interest in simpler methods like momentum SGD as they may yield better test metrics. Motivated by this trend, we ask: can simple adaptive methods based on SGD perform as well or better? We revisit the momentum SGD algorithm and show that hand-tuning a single learning rate and momentum makes it competitive with Adam. We then analyze its robustness to learning rate misspecification and objective curvature variation. Based on these insights, we design YellowFin, an automatic tuner for momentum and learning rate in SGD. YellowFin optionally uses a negative-feedback loop to compensate for the momentum dynamics in asynchronous settings on the fly. We empirically show that YellowFin can converge in fewer iterations than Adam on ResNets and LSTMs for image recognition, language modeling and constituency parsing, with a speedup of up to 3.28x in synchronous and up to 2.69x in asynchronous settings.

==> misc.tex <==
\section{Misc}


\begin{lemma}
	Let the $h$ be the curvature of quadratic function $f$. With $\overline{x}_t$ being the expectation of $x_t$, we assume, without loss of generality, the optimum point of the quadratic $f$ is 0. Then we have the following recurrence
	\begin{equation} 
		\begin{pmatrix}
			\overline{x}_{t + 1} \\
			\overline{x}_t
		\end{pmatrix} = 
		\begin{pmatrix}
			1-\alpha h + \mu & - \mu\\
			1 & 0 \\
		\end{pmatrix}
		\begin{pmatrix}
			\overline{x}_1 \\
			\overline{x}_0
		\end{pmatrix}
	\end{equation} 
\end{lemma}

\begin{lemma}
	We define $U_t=\E \| x_t - \overline{x}_t \|^2$ and $V_t= \E (x_t - \overline{x}_t) (x_{t-1} - \overline{x}_{t-1})$ with $\overline{x}_t$ being the expectation of $x_t$. For quadratic function $f(x)$ with curvature $h \in \mathbb{R}$, We have the following recurrence
	\begin{equation} 
		\begin{pmatrix}
			U_{t+1} \\
			U_t \\
			V_{t + 1}
		\end{pmatrix} = 
		(\mat{I} - \mat{S}^T)(\mat{I} - \mat{S})^{-1}
		\begin{pmatrix}
			\alpha^2 \\
			0 \\
			0
		\end{pmatrix}
	\end{equation}
	where 
	\begin{equation}
		\mat{S} = 
		\begin{pmatrix}
		(1-\alpha h + \mu)^2 &  \mu^2 & -2\mu(1-\alpha h + \mu)\\
		1 & 0 & 0 \\
		1-\alpha h + \mu & 0 & - \mu
		\end{pmatrix}
	\end{equation}
\end{lemma}


\begin{lemma}
\label{lem:2times2_spectral_radius}
	Let $\rho(\mat{T})$ be the spectral radius of matrix  
\begin{equation}
	\mat{T} = \begin{pmatrix}
	1-\alpha h + \mu & - \mu\\
	1 & 0 \\
	\end{pmatrix}
\end{equation}
where $h\in \mathbb{R}$. $\rho(\mat{T}) = \sqrt{\mu}$ if the following condition holds
\begin{align}
{(1-\sqrt{\mu})^2\over \alpha} &\leq h \leq {(1+\sqrt{\mu})^2\over \alpha}.
\label{equ:control_condition_scalar}
\end{align}
\end{lemma}

\begin{lemma}
\label{lem:3times3_spectral_radius}
Let $\rho(\mat{S})$ be the spectral radius of matrix 
\begin{equation}
	%\rho_V(\alpha, \mu) = \rho \left(
\mat{S} = {\begin{pmatrix}
(1-\alpha h + \mu)^2 &  \mu^2 & -2\mu(1-\alpha h + \mu)\\
1 & 0 & 0 \\
1-\alpha h + \mu & 0 & - \mu
\end{pmatrix}}
	%\right)
\end{equation}
where $h\in \mathbb{R}$.
$\rho(\mat{S})=\mu$ if the following condition holds for
\begin{equation}
{(1-\sqrt{\mu})^2\over \alpha} \leq h \leq {(1+\sqrt{\mu})^2\over \alpha}
\label{equ:control_condition_var}
\end{equation}
\end{lemma}



\begin{corollary}
\label{cor:}
Under the conditions in Eqaution~\eqref{equ:control_condition_var}, we get
\begin{equation}
	\E \| x_T \|^2 
	= \mu^T \| x_0 \|^2
		+ (1-\mu^T) \frac{\alpha^2 C}{1-\mu}
	\label{equ:noisy_square_dist}
\end{equation}
\label{cor:noisy_dist}
\end{corollary}

Now, if we know, or can approximately estimate some of these quantities we can tune the learning rate and momentum hyperparameters to minimize  \eqref{equ:noisy_square_dist}.





\section{Proof of Lemma~\ref{}}
The generalization of scalar analysis to multiple dimensional case.
\begin{lemma}
\label{lem:robustness}
Let the gradients of a function $f$ be described by
\begin{equation}
	\nabla f(\mat{x}_t) = \mat{H}_t (\mat{x}_t - \mat{x}^*),
\end{equation}
for $\mat{H}_t \in \mathbb{R}^{n\times n}$.
The the momentum update can be expressed as a linear operator:
\begin{align}
{\begin{pmatrix}
\mat{y}_{t+1}\\
\mat{y}_t \\
\end{pmatrix}}
=
{\begin{pmatrix}
\mat{I}-\alpha \mat{H}_t + \mu \mat{I} & - \mu \mat{I} \\
\mat{I} & \mat{0} \\
\end{pmatrix}}
{\begin{pmatrix}
\mat{y}_t \\
\mat{y}_{t-1} \\
\end{pmatrix}}
=\mat{T}_t
{\begin{pmatrix}
\mat{y}_t \\
\mat{y}_{t-1} \\
\end{pmatrix}},
\end{align}
where $\mat{y}_t\triangleq \mat{x}_t - \mat{x}^*$.
Now, assume that the following condition holds for all eigenvalue $\rho(\mat{H}_t)$ of $\mat{H}_t$ for all $t$:
\begin{align}
{(1-\sqrt{\mu})^2\over \alpha} &\leq \rho(\mat{H}_t ) \leq {(1+\sqrt{\mu})^2\over \alpha}.
\label{equ:control_condition}
\end{align}
then the spectral radius of $\mat{T}_t$ is controlled by momentum with
$	\rho(\mat{T}_t) = \sqrt{\mu}.$

\begin{proof}
Let $\lambda_t$ be an eigenvalue of matrix $\mat{T}_t$, it gives 
$\det\left(\mat{T}_t - \lambda_t \mat{I} \right) = 0$. 
We define $\mat{A}_t = \mat{I} - \alpha \mat{H}_t + \mu \mat{I} - \lambda_t \mat{I}$, $\mat{B}_t = -\mu \mat{I}$,
$\mat{C}_t = \mat{I}$ and $\mat{D}_t = -\lambda_t \mat{I}$ which gives
\[
\det \left( \mat{T}_t - \lambda_t \mat{I}\right) = \det{\mat{D}_t} \det{\left(\mat{A}_t - \mat{B}_t \mat{D}_t^{-1}
\mat{C}_t \right)} = 0
\]
assuming generally $\mat{D}_t$ is invertable. The equation $\det{\left(\mat{A}_t - \mat{B}_t \mat{D}_t^{-1}
\mat{C}_t \right)} = 0$ implies that
\begin{equation}
\det \left( \lambda_t^2\mat{I} - \lambda_t \mat{M}_t + \mu \mat{I} \right) = 0
\label{equ:control_condition_2}
\end{equation}
with $\mat{M}_t = \left( \mat{I} - \alpha \mat{H}_t + \mu \mat{I} \right)$. In other words, $\lambda_t$ satisfied that $\lambda_t^2 - \lambda_t \rho(\mat{M}_t) + \mu = 0$ with $\rho(\mat{M}_t)$ being one eigenvalue of $\mat{M_t}$. I.e.
\begin{equation}
	\lambda_t = \frac{\rho(\mat{M}_t) \pm \sqrt{\rho(\mat{M}_t)^2 - 4\mu}}{2}
\end{equation}

On the other hand, Equation~\eqref{equ:control_condition} guarantees that $(1 - \alpha \rho(\mat{H}_t) + \mu)^2 \leq 4\mu$. We know both $\mat{H}_t$ and $\mat{I} - \alpha \mat{H}_t + \mu \mat{I}$ are symmetric. Thus for all eigenvalues $\rho(\mat{M}_t)$ of $\mat{H}$, we have $\rho(\mat{M}_t) = (1 - \alpha \rho(\mat{H}_t) + \mu)^2 \leq 4\mu$ which guarantees $| \lambda_t | \leq \sqrt{\mu}$ for all $\lambda_t$ and all $t$. As the spectral radius is equal to the absolute value of the largest eigenvalue of $\mat{T}_t$, we have the spectral radius of $\mat{T}_t$ is $\sqrt{\mu}$ for all $t$.


\end{proof}
	
\end{lemma}


\begin{corollary}
	Let the gradients of a function $f$ be described by
\begin{equation}
	\nabla f(x_t) = h_t (x_t - x^*),
\end{equation}
for $h_t \in \mathbb{R}$.
The the momentum update can be expressed as a linear operator:
\begin{align}
{\begin{pmatrix}
y_{t+1}\\
y_t \\
\end{pmatrix}}
=
{\begin{pmatrix}
1-\alpha h_t + \mu & - \mu\\
1 & 0 \\
\end{pmatrix}}
{\begin{pmatrix}
y_t \\
y_{t-1} \\
\end{pmatrix}}
=\mat{T}_t
{\begin{pmatrix}
y_t \\
y_{t-1} \\
\end{pmatrix}},
\end{align}
where $y_t\triangleq x_t - x^*$.
Now, assume that the following condition holds for all $t$:
\begin{align}
{(1-\sqrt{\mu})^2\over \alpha} &\leq h_t \leq {(1+\sqrt{\mu})^2\over \alpha}.
\label{equ:control_condition_scalar}
\end{align}
then the spectral radius of $\mat{T}_t$ is controlled by momentum with
$	\rho(\mat{T}_t) = \sqrt{\mu}.$
\end{corollary}

\begin{lemma}
Let $\rho(\mat{S})$ be the spectral radius of matrix 
\begin{equation}
	%\rho_V(\alpha, \mu) = \rho \left(
\mat{S} = {\begin{pmatrix}
(\mat{I}-\alpha \mat{H} + \mu \mat{I})^T(\mat{I}-\alpha \mat{H} + \mu \mat{I}) &  \mu^2 \mat{I} & -2\mu(\mat{I}-\alpha \mat{H} + \mu \mat{I})\\
\mat{I} & \mat{0} & \mat{0} \\
\mat{I}-\alpha \mat{H} + \mu \mat{I} & \mat{0} & - \mu \mat{I} 
\end{pmatrix}}
	%\right)
\end{equation}
$\rho(\mat{S})=\mu$ if the following condition holds for all eigenvalues $\rho(\mat{H})$ of $\mat{H}\in \mathbb{R}^{n \times n}$
\begin{equation}
{(1-\sqrt{\mu})^2\over \alpha} \leq \rho(\mat{H}) \leq {(1+\sqrt{\mu})^2\over \alpha}
\label{equ:control_condition_var}
\end{equation}

\begin{proof}
	Let $\lambda$ be an eigenvalue of matrix $\mat{S}$, it gives 
$\det\left(\mat{S} - \lambda \mat{I} \right) = 0$ which can be alternatively expressed as
\begin{equation}	
\det \left( \mat{S} - \lambda \mat{I}\right) = \det{\mat{D}} \det{\left(\mat{A} - \mat{B} \mat{D}^{-1}
\mat{C} \right)} = 0
\label{equ:control_condition_var_1}
\end{equation}
assuming $\mat{D}$ is invertible, i.e. $\lambda + \mu \neq 0$, where \begin{equation*}
		\mat{A} = \left( { \begin{array}{c c}
 			\mat{M}^T\mat{M} - \lambda \mat{I} &  \mu^2 \mat{I} \\
 			\mat{I} & - \lambda \mat{I}
 		\end{array} } \right), 
 		\mat{B} = \left( { \begin{array}{c}
 			-2\mu \mat{M} \\
 			\mat{0}
 		\end{array}}\right),
 		\mat{C} = \left( {\begin{array}{c}
 			\mat{M} \\
 			\mat{0}
 		\end{array}} \right)^T,
 		\mat{D} = -\mu \mat{I} - \lambda \mat{I}
	\end{equation*}
	with $\mat{M}=\mat{I}-\alpha \mat{H} + \mu \mat{I}$. It can be transformed using straight-forward algebra as
	\begin{equation}
		\det \left( \begin{array}{c c}
 			(\lambda - \mu) \mat{M}^T\mat{M} - (\lambda + \mu) \lambda \mat{I} & (\lambda + \mu)\mu^2 \mat{I} \\
 			(\lambda + \mu) \mat{I} & -(\lambda + \mu)\lambda \mat{I}
 		\end{array} \right)
		\label{equ:control_condition_var_2}	
	\end{equation}
	Using similar simplification technique as in Equation~\eqref{equ:control_condition_var_1}, we can further simplify into
	\begin{equation}
		(\lambda - \mu)\det \left( (\lambda + \mu)^2 \mat{I} - \lambda \mat{M}^T\mat{M} \right) = 0
	\end{equation}
	if $\lambda \neq \mu$, as $(\lambda + \mu)^2 \mat{I} - \lambda \mat{M}^T\mat{M}$ is diagonalizable, we have $(\lambda + \mu)^2 - \lambda \rho(\mat{M})^2 = 0$ with $\rho(\mat{M})$ being an eigenvalue of $\mat{M}$. The analytic solution to the equation can be explicitly expressed as
	\begin{equation}
		\lambda = \frac{\rho(\mat{M})^2 - 2\mu \pm \sqrt{(\rho(\mat{M})^2 - 2\mu)^2 - 4\mu^2}}{2}
		\label{equ:control_condition_var_3}	
	\end{equation}.
	
	When the condition in Equation~\eqref{equ:control_condition_var} holds, we have $(1 - \alpha \rho(\mat{H}_t) + \mu)^2 \leq 4\mu$. One can verify that 
	
	\begin{equation}
		\begin{aligned}
			(\rho(\mat{M})^2 - 2\mu)^2 - 4\mu^2 & = && (\rho(\mat{M})^2 - 4\mu)\rho(\mat{M})^2 \\
			& = &&\left( (1 - \alpha \rho(\mat{H} ) + \mu)^2 - 4\mu\right)\rho(\mat{M})^2 \\
			& \leq && 0
		\end{aligned}
	\end{equation}
	Thus the roots in~\eqref{equ:control_condition_var_3} are conjugate and we have $| \lambda | = \mu$. In conclusion, the condition in Equation~\eqref{equ:control_condition_var} can guarantee all the eigenvalues of $\mat{S}$ has magnitude $\mu$. Thus the spectral radius of $\mat{S}$ is controlled by $\mu$
\end{proof}

\end{lemma}

\begin{corollary}
	
Let $\rho(\mat{S})$ be the spectral radius of matrix 
\begin{equation}
	%\rho_V(\alpha, \mu) = \rho \left(
\mat{S} = {\begin{pmatrix}
(1-\alpha h + \mu)^2 &  \mu^2 & -2\mu(1-\alpha h + \mu)\\
1 & 0 & 0 \\
1-\alpha h + \mu & 0 & - \mu
\end{pmatrix}}
	%\right)
\end{equation}
where $h\in \mathbb{R}$.
$\rho(\mat{S})=\mu$ if the following condition holds for
\begin{equation}
{(1-\sqrt{\mu})^2\over \alpha} \leq h \leq {(1+\sqrt{\mu})^2\over \alpha}
\label{equ:control_condition_var}
\end{equation}

\end{corollary}

\begin{theorem}
refer to the main content to theorem 2. \textbf{We need to assume quadratic in this theorem}
\begin{proof}
	From the recurrence of momentum SGD, we have $x_{t+1} = x_t - \alpha \nabla f_{S_t} (x_t) + \mu (x_t - x_{t-1})$. And the expected squared distance to the optimal point can be decomposed as $\E \| x_t - x^* \|^2 = \E \| x_t - \overline{x}_t \|^2 + \| \overline{x}_t- x^* \|^2$, where $\overline{x}_t$ is the expectation of $x_t$.
	Without loss of generality, we assume the optimum $x^*=0$ and investigate the bias term $\| \overline{x}_t- x^* \|^2$ and variance term $\E \| x_t - \overline{x}_t \|^2$ respectively.
	
	For the bias term, we have $\| \overline{x}_{t + 1} \|^2 = \| \overline{x}_t - \alpha \nabla f( \overline{x}_t) + \mu ( \overline{x}_t -  \overline{x}_{t - 1})\|^2$
	\begin{equation}
		\left(\begin{array}{c}
		 \overline{x}_{t+1} \\
		 \overline{x}_{t}	
		\end{array}\right) =
		\left(\begin{array}{c c}
			1 - \alpha h_t + \mu & - \mu \\
			1 & 0
		\end{array}\right)
		\left(\begin{array}{c}
		 \overline{x}_{t} \\
		 \overline{x}_{t-1}	
		\end{array}\right)
	\end{equation}
	
	For the variance term recurrence, we have $\nabla f(x_t) = h x_t$ 
	\begin{equation}
		\begin{aligned}
			\E \| x_{t + 1} - \overline{x}_{t + 1} \|^2 = \E \| x_{t} - \alpha \nabla f_{S_t}(x_t) + \mu (x_{t} - x_{t - 1})
				- \overline{x_t} + \alpha \nabla f(\overline{x}_t) - \mu (
				\overline{x}_t - \overline{x}_{t - 1}) \|^2 
		\end{aligned}
	\end{equation} 
\end{proof}

\end{theorem}









==> tmp.tex <==
\section{Introduction}

\begin{itemize}
\item Tuning is important in deep learning and tuning is hard.
\item People do (a) adaptive (b) method with knob. (Fix momentum and only investigate lr).
\item momentum accelerates. better understanding the behavior of momentum is interesting better tuner with less tuning. We revisit mom sgd and found the robustness to lr and variation. As well as related to async. And derive simple theory to analyze. 
\item These properties makes mom sgd a good candidate for auto tuning. We investigate a quadratic model and propose an simple and easy to understand tuner. It is faster than Adam
\item We also connect to async theory and develope component and better than others in asynchrony.  
\end{itemize}

\outline{[PROBLEM]}
Deep learning involves the use of very large datasets to fit large, complex models.
Accelerated forms of stochastic gradient descent (SGD), pioneered by
\cite{polyak1964some} and \cite{nesterov1983method}, are the de-facto
algorithms for training deep nets.
Using those optimization methods requires a sane choice for their {\em hyperparameters}: 
typically a {\em learning rate} and {\em momentum parameter} \citep{sutskever2013importance}.
Furthermore, the scale of the typical deep learning problem, implies a computationally heavy optimization procedure and motivates parallelization \cite{dean2012large,chilimbi2014project,hadjis2016omnivore,chen2016revisiting}.
Asynchronous methods \cite{recht2011hogwild} provide very efficient parallelization by doing away with locking and synchronization. 
Recent work \cite{mitliagkas2016asynchrony,hadjis2016omnivore} shows that proper {\em tuning} of the momentum hyperparameter is important for achieving good asynchronous performance as {\em asynchrony introduces an extra momentum term}.

\outline{[IMPORTANT AND HARD]}
Hyperparameter tuning is often cited as being the number-one factor in extracting good performance from deep learning systems. 
It is by far the most time consuming phase of developing a new deep learning model or system.
One could say that tuning is {\em the hidden cost of modern machine learning},
with thousands of grad-student-hours sacrificed and many papers outlining best practices written
\cite{bengio2012practical}.
Na\"ive methods, like grid-searching the hyperparameter values,
is prohibitively expensive for all but the smallest models and datasets.


\outline{[PREVIOUS APPROACHES]}
Deep learning researchers have proposed a number of methods to deal with hyperparameter tuning. 
Black box methods like random search \cite{bergstra2012random} and
derivative-free optimization approaches (eg.\ Bayesian) \cite{snoek2012practical}
do not take into account the dynamics of the problem and might need to run many time consuming evaluation trials.
Adaptive methods provide an attractive option and have been largely successful in relieving practitioners of the burden of tuning the learning rate parameter. 
Algorithms like Adagrad \cite{duchi2011adaptive}, RMSProp \cite{tieleman2012lecture}, Adam \cite{kingma2014adam} use the magnitude of gradient elements to tune learning rate {\em individually for each variable}.
Finally, methods like the one proposed in \cite{schaul2013no} use a simple model and simple measurements to tune a global learning rate for the standard SGD update.
A common limitation for the state of the art, is that none of the available adaptive algorithms tunes its momentum parameter,\footnote{Some do not use acceleration at all.}
an important factor for both synchronous and asynchronous performance.


\begin{wrapfigure}[14]{R}{0.5\textwidth}
\vspace{-2em}
\begin{minipage}{1.0\linewidth}
\begin{figure}[H]
	\includegraphics[width=1.0\linewidth]{experiment_results/spotlight.pdf}
	\caption{\tuner in comparison to Adam.}
\end{figure}
\end{minipage}
\end{wrapfigure}
We revisit the simple momentum SGD algorithm and propose \tuner, an automatic tuner for its hyperparameters.
A key component of \tuner is principled momentum-tuning in both synchronous and asynchronous settings.
\tuner is competitive or better that state-of-the-art adaptive methods and is asynchrony-aware by using a novel design based on measuring the level of momentum on the fly and using a closed-loop control module for momentum.

\outline{[OUR RESULTS]}
We demonstrate experimentally, in Section~\ref{sec:experiments}, that
for a large class of networks, hand-tuned momentum SGD is competitive with Adam ($0.88-1.82\times$), even though it uses fixed hyperparameters throughout execution.
On ResNets, momentum SGD can achieve a $1.25-1.82\times$ speedup over Adam.
\tuner is competitive with, and sometimes better, than state-of-the-art adaptive methods. The speedup is over $2\times$ on ResNets and $1.18\times$ on LSTMs.
Other adaptive algorithms do not tune their momentum parameter and suffer, as a result, in asynchronous settings.
Hand-tuning momentum for Adam can improve its convergence rate by up to $2\times$, when using $16$ asynchronous workers. 
Finally, closing the momentum loop in \tuner yields a speedup of $1.3-3\times$, when using $16$ asynchronous workers.
Closed-loop \tuner achieves a speedup of about $2.7\times$ over Adam on 16 asynchronous workers.


